How Far Does BERT Look At:Distance-based Clustering and Analysis of BERT$'$s Attention

Recent research on the multi-head attention mechanism, especially that in pre-trained models such as BERT, has shown us heuristics and clues in analyzing various aspects of the mechanism. As most of the research focus on probing tasks or hidden states, previous works have found some primitive patterns of attention head behavior by heuristic analytical methods, but a more systematic analysis specific on the attention patterns still remains primitive. In this work, we clearly cluster the attention heatmaps into significantly different patterns through unsupervised clustering on top of a set of proposed features, which corroborates with previous observations. We further study their corresponding functions through analytical study. In addition, our proposed features can be used to explain and calibrate different attention heads in Transformer models.

==> fig/src/ablation.tex <==
\section{Attention Ablation} \label{sec:ablation}

We start to explore attention behavior according to distance with several direct ablation experiments.
Firstly, we prune attention heads or substitute them with uniformed attention to find out their importance to the BERT model.
Then, we constrain the distance of attention heads to see which part of information is utilized by each type.
This is implemented by ablating attention with sentence granularity.

\subsection{Pruning and Substitution} \label{sec:ablation:pruning}

\citet{?,?,?} have shown that MHA mechanism is overparameterized.
About $30\%$ of heads are pruned without any influence to model's normal processing and accuracy.
Our question is, are there importance difference in attention behaviors.
And for the dense pattern, attention values at different positions are very close. \fixme{need data here}
% When the input sequence is long, for instance 512 is a normal setting for BERT-large, the slight divergence at each position have few influence to the output embedding.
As such, are these dense values immutable?
We answer these questions by pruning attention heads or substituting them with uniformed attention.

\textbf{Setup: }
We make the pruning experiment following \citep{}, except we are not using a pre-trained BERT language model.
Accuracy and F1 are evaluated as metrics for the question and answering task.
While testing on SQUAD development set, the attention matrix is either set to zeros matrix or uniformed attention of $1/L$.
As such, a head is either pruned or substituted.
% Because pruning single or few heads have negligible effect on the model, all heads are substituted together.

\textbf{Results: }Results are shown as \Tbl{tbl:pruning_ablation}.
We first find that pruning all \benchmark{vertical} type heads has nearly no influence.
% This result is consistent to the probing tasks results.
This means the output embeddings of this type have limited influence to the model processing.
According to our clustering result, such \benchmark{vertical} type makes up roughly $15.6\%$ of total number.
Although there are $27.6\%$ of \benchmark{dense} heads, pruning them all has a surprisingly low performance influence to the model, less than $5\%$.
We suppose this is because its functions are covered by other types.
This function duplication between heads is another reason for the redundancy.

For all cases, substituting a head has larger interference than pruning it.
Even so, the model remains nearly $70\%$ accuracy when all \benchmark{dense} types are substituted by uniformed attention.
This result suggests that the attention values of \benchmark{dense} are not immutable.
Finally, for both experiments, changing \benchmark{diagonal} type heads makes model nonfunctional.
It indicates that \benchmark{diagonal} type is important and its function is not intersected with other types.


\subsection{Ablation by Distance}
Following the observation that attention behaviors correspond to information at different distance, we design direct ablation experiments to control attention according to distance.
We use sentences as native boundary and ablate either attention intra-sentence or inter-sentence.
When intra-sentence attention are ablated, such attention head only has access to tokens in other sentences and obtains global information.
On the contrast, when inter-sentence attention are ablated, attention head has only local syntactic or word level semantic information.
Our purpose is to find out which kind of information is important for each head.

\textbf{Setup: } 
The setting is similar to which has been introduced in \Sec{sec:ablation:pruning}.
Instead of pruning the whole attention head, blocks are ablated by sentences as shown in \Fig{fig:ablation_schematic}.
In case the question sentence is not 'understood' properly, attention inside the question sentence is never ablated.

We present two ablation schemes ablate-one and leave-one-out.
\Fig{fig:ablation_schematic} is an example of the two schemes with \benchmark{diagonal} type as target.
Ablate-one means only the target type is ablated, measuring how much information is lost when such type is absent.
Leave-one-all means all the other types are ablated except for the target one, measuring how much information is passes by this particular type.

\textbf{Results: } 
\Fig{fig:ablation_result} shows the results.
For ablate-one scheme, all types of attention heads achieved a descent result when ablated either intra-sentence or inter-sentence attention, except for diagonal sentence under intra-sentence ablation setting.
This is explained by that both global and local information are handled by different types of heads.
Only the \benchmark{diagonal} type plays an inevitable role dealing with intra-sentence attention.
When it is absent, model accuracy drops significantly to $14.01\%$.

For leave-one-out scheme, performance of the model is damaged badly.
Because only few attentions heads remains to process the information and this is quite hard a constrain.
However, we still find three cases where the model still predicts the correct answers.
They are when \benchmark{diagonal} type remains intra-sentence attention and \benchmark{dense} or \benchmark{dense\&vertical} type remains inter-sentence attention.
This phenomenon shows that such kind of information is processed properly with only the particular type.
For example, only \benchmark{dense\&vertical} type heads attending inter-sentence tokens reaches $74.84\%$ accuracy, which is less than $10\%$ loss comparing with the native model. 

% \begin{figure}[h] \label{fig:ablation_schematic}
%   \includegraphics[width=\columnwidth]{fig/ablation_schematic.png}
%   \caption{explanation of ablation experiment setup. \fixme{to be re-drawed}}
% \end{figure}

\begin{table*}[]
  \begin{tabular}{|c|c|c|c|c|c|}
  \hline
  \multicolumn{2}{|c|}{}                                                                                         & \small \benchmark{Dense} & \small \benchmark{Diagonal} & \tiny \benchmark{Dense\&Vertical} &\small \benchmark{Vertical} \\ \hline
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\small Ablate-one\\ \end{tabular}}    & Intra & \cmark              & \xmark                 & \cmark                        & \cmark                 \\ \cline{2-6} 
                                                                                                         & Inter & \cmark              & \cmark                 & \cmark                        & \cmark                 \\ \hline
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\tiny Leave-one-out\\ \end{tabular}} & Intra & \xmark              & \cmark                 & \xmark                        & \xmark                 \\ \cline{2-6} 
                                                                                                         & Inter & \cmark              & \cmark                 & \cmark                        & \cmark                 \\ \hline
  \end{tabular}
  \caption{ablation schemes example of setting diagonal and intra-sentence.}
\end{table*}

\begin{table*}[]
  \begin{tabular}{cccccccccc}
    \hline
    \multicolumn{2}{c}{\multirow{2}{*}{}}  & \multicolumn{2}{c}{\textbf{Dense}} & \multicolumn{2}{c}{\textbf{Diagonal}} & \multicolumn{2}{c}{\textbf{dense\&vertical}} & \multicolumn{2}{c}{\textbf{Vertical}} \\ 
    \multicolumn{2}{c}{}                   & Acc.(\%)   & F1(\%)   & Acc.(\%)     & F1(\%)    & Acc.(\%)          & F1(\%)         & Acc.(\%)     & F1(\%)    \\ \hline
    \multicolumn{2}{c}{Number}             & \multicolumn{2}{c}{100}   & \multicolumn{2}{c}{102}       & \multicolumn{2}{c}{131}                 & \multicolumn{2}{c}{51}       \\ \hline
    \multicolumn{2}{c}{Baseline}           & \multicolumn{8}{c}{82.85 / 89.68}                                                                                                  \\\hline\hline
    \multicolumn{2}{c}{Substitution}       & 69.77          & 80.00    & \textit{1.44}             & \textit{6.30}      & 14.95                 & 18.08          & 53.17            & 59.09     \\
    \multicolumn{2}{c}{Pruning}            & 78.17          & 86.40    & \textit{2.47}             & \textit{4.23}      & 66.72                 & 76.11          & 82.16            & 89.24     \\ \hline\hline
    \multirow{2}{*}{Ablate-all}    & Intra & \multicolumn{8}{c}{4.08 / 8.92}                                                                                                    \\
                                   & Inter & \multicolumn{8}{c}{12.12 / 19.9}                                                                                                   \\ \hline
    \multirow{2}{*}{Ablate-one}    & Intra & 79.21          & 87.01    & 82.01            & 89.00     & 74.32                 & 82.76          & 82.59            & 89.47     \\
                                   & Inter & 82.4           & 89.36    & \textit{14.01}            & \textit{20.97}     & 79.99                 & 87.41          & 82.64            & 89.55     \\ \hline
    \multirow{2}{*}{\small Leave-one-out} & Intra & 13.44          & 21.99    & \textit{71.89}            & \textit{80.47}     & 14.21                 & 22.61          & 13.5             & 22.10     \\
                                   & Inter & \textit{65.62}          & \textit{75.06}    & 10.73            & 16.26     & \textit{74.84}                 & \textit{83.43}          & 9.21             & 15.45     \\ \hline
    \end{tabular}
    \caption{Pruning and ablation experiments result}
    \label{table:pruning_ablation}
\end{table*}


% \begin{figure}[h] \label{fig:ablation_result}
%   \includegraphics[width=\columnwidth]{fig/ablation_result.png}
%   \caption{explanation of ablation experiment setup.}
% \end{figure}

==> fig/src/probing.tex <==
\section{Probing Tasks} \label{sec:probing}

% \textbf{Outlint: }
% Introduce the experiment setup of dependency parsing and QNLI.
% We use attention instead of embedding to build connection with behavior pattern.
% We use multiple sentences task to explore the head function dealing with global sematic information.

We have shown what kind of information each attention behavior type handles in \Sec{sec:ablation}.
To further understand the connection between direct distance and linguistic hierarchy, we performed several probing tasks in this section.
A probing task is a classification problem used to detect linguistic properties \citep{?}.
We design probing tasks with attention matrix to find out the linguistic information encoded by the behavior patterns mentioned in this paper.

\subsection{Experiment Setup} \label{probing:setup}

We introduce the setup of two types of probing tasks with attention weight matrix.
Dependency parsing problem is used for intra-sentence probing.
And novel probing task innovated by QNLI task \citep{?} measures inter-sentence semantic capability.

\subsubsection{Intra-Sentence Probing}

Dependency parsing problem is a common downstream problem of NLP \citep{?}.
It is to generate the linguistic dependency relations given input sentence.
There have been works using it as a probing task to study interpretability of MHA \citep{?,?}.
Comparison to these works will be discussed in \Sec{sec:related}.

We extract the attention matrix from BERT-large model as input for the probing task.
% That is to detect the syntactic information enclosed in MHA.
Universal dependency \citep{?} tags are annotated with the Stanza \citep{?} library on SQUAD dataset.
We select the most frequent 12 dependency relations and others as negative samples.
Classes are down-sampled to keep the problem balanced.
Then it forms a 13-classes classification problem given the attention value between two words.
We used annotated samples from SQUAD training set to fit a simple multi-layer perceptron (MLP) model \citep{} and report the evaluation accuracy on annotated SQUAD development set.

Furthermore, BERT model takes sub-word level tokens as input.
To reproduce the word attention, we follow the processing of \citep{} to accumulate word attention.
And the accumulation method is generalized into regional attention as Eq.~\ref{?}, which will be used at sentence level in \Sec.{sec:probing:qnli}.
\begin{equation} \label{equ:region_attention}
  \small \underset{\{from [m,n], to [s,t]\}}{RegionAttention}=\frac{1}{t-s}\sum_{i=s}^t(\sum_{j=m}^n{Attention(x_i,x_j)})
\end{equation}
For dependency parsing problem discussed here, region is defined as tokens split from a word.
Another setting is that we use not only the attention to the target word, but also the attention to special token '[CLS]' and '[SEP]'.
This is based on the observation in \Sec{sec:clustering:clustering} that many heads have attention to these tokens. 

\subsubsection{Inter-Sentence Probing} \label{sec:probing:qnli}
% \textbf{Outline} To predict sentence whether containing answer as QNLI task.
% Layer-wise result of QNLI probing.
% High-level sematic information are synthesized gradually.
% Top layers have the highest accuracy.
% We can find out whether a sentence containing result by the attention behavior.

Motivated by the QNLI task \citep{}, we design a novel probing task to detect semantic property at sentence level.
Paragraphs in QNLI dataset is the same as SQUAD question answering task.
However, instead of producing an answer prediction, QNLI is a classification problem of finding whether a sentence containing the correct answer.
As so, we can use similar target task to check whether the BERT-large model on SQuAD finds out the position of the answer.
And the idea is simple, if model locates the answer, the attention between question and answer sentence must be distinguishable.

We calculate the attention between sentences as Eq.~\ref{equ:region_attention}.
Similarly, attention to the special tokens are taken into consideration separately.
We evaluate such attention relations and set binary classification target as containing answer.
As there exists multiple questions for one paragraph in SQUAD dataset, we randomly pick one question to avoid repeating sentence pairs.
Again, the training set and development set are used to fit and evaluate a MLP model.


\subsection{Results}
% \textbf{Outline} The overall results of both probing tasks of different head type.
% Build the connection between attention behavior and function.

We report the probing tasks results by layers and by head types respectively.

\subsubsection{By layers.}
The results are first reported by layers as \Fig{fig:parsing_layer}.
It is surprising that the QNLI probing task reaches accuracy over $80\%$ at the first layer.
This means that BERT-large model managed to locate the answer with input embeddings and positional embeddings barely.
For example, by finding same or similar key words in question sentence, sentence containing answer is recognized.
The QNLI probing accuracy increases as layer getting higher.

On the contrast, accuracy of dependency parsing is stable at bottom layers and drops at last layers.
We further breakdown the accuracy of each dependency relation class and show two representative ones for simplicity.
Results of other dependencies are similarly and don't change any analysis in this section, which can be found in Appendix~\ref{}.
We find surface level dependencies such as 'det' have highest probing accuracies at bottom layers.
Dependencies of more abstract relations reaches highest probing accuracies at middle layers.
Similar conclusion is reported by \citet{?} with probing task utilizing contextual embeddings.
However, what is the reason for this phenomenon?
Our experiments in next section shows it is caused by the distribution of attention types.

\begin{figure}[h]
  \includegraphics[width=\columnwidth]{fig/dependency_parising_layer_wise.pdf}
  \caption{dependency parsing layer wise result.\fixme{multiple times and deviation}}
  \label{fig:parsing_layer}
\end{figure}


\subsubsection{By head types.}
Dependency parsing probing task results by head types are shown with \Fig{fig:parsing_type}.
We calculated the average distance of each linguistic relation and arrange \Fig{fig:parsing_type} according to it.
Special cases are 'nummod', 'advmod' and 'compound', whose average distance is less than 1.
It is because they appears on both sides of the source word in sentence, unless most other relations having their target whether before or behind the source word.

For short distance relations such as 'det', \benchmark{dense} type has the highest probing accuracy.
For relations with longer distance, \benchmark{diagonal} type outperforms other types.
\benchmark{Vertical} type heads have the lowest accuracy on nearly all relations.

QNLI probing results are shown with \Fig{fig:parsing_type_qnli}.
% Results are shown of each head instead of each type.
% Because we find all types have decent and close results with all heads.
Generally, \benchmark{dense\&vertical} types have higher accuracies in all layers than other types.
This is consistent with intuition because the dense pattern attentions to global information with long distance.
And \benchmark{diagonal} are the worse ones in each layers.
Most \benchmark{dense} heads don't seems to be capable of identifying the correct answer sentence.
However, few this type heads have accuracy near $80\%$ suggesting they are finding key words according to question.
For \benchmark{vertical} type heads, most of this type heads are the worst at each layer.
But there do exist part of \benchmark{vertical} heads having the best performance.
Even though, our experiments in \Sec{sec:ablation:ablation} indicate that they are not critical.

As such, we describe a general view of the MHA.
Most heads at bottom layers are \benchmark{dense} type.
They handle the surface level syntactic information.
\benchmark{Diagonal} heads distribute across all layers and deals with intra-sentence semantic information.
\benchmark{dense\&vertical} heads are mainly in middle layers and deals with global information.
It is stressed here this conclusion doesn't mean such heads only do that particular job.
Results show that \benchmark{dense\&vertical} heads also have compatible performance on many dependency relations.
\benchmark{Vertical} type at top layers have poor performance on all levels of probing tasks.


\begin{figure}[h]
  \includegraphics[width=\columnwidth]{fig/parsing_type.pdf}
  \caption{dependency parsing type wise result. }
  \label{fig:parsing_type}
\end{figure}

\begin{figure}[h]
  \includegraphics[width=\columnwidth]{fig/probing_type_wise.pdf}
  \caption{probing result type wise result.}
  \label{fig:parsing_type_qnli}
\end{figure}


==> section/preamble.tex <==
% to be able to draw some self-contained figs
\usepackage{tikz}
\usepackage{mathptmx} % This is Times font

%\usepackage{subfig}
\usepackage{amsmath}
\usepackage[normalem]{ulem}
\usepackage{amssymb}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{pifont}
\usepackage[noend]{algorithmic}
\usepackage[ruled, linesnumbered]{algorithm2e}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{color}
\usepackage{listings}
\usepackage{float}
\usepackage{ragged2e}
\usepackage{xspace}
\usepackage{soul}
\usepackage{lipsum}
\usepackage{makecell}
\usepackage{mathtools}
\usepackage{subcaption}
\usepackage{fancyhdr}
\usepackage[normalem]{ulem}
\usepackage[hyphens]{url}
\usepackage[sort,nocompress]{cite}
\usepackage[final]{microtype}
\usepackage[keeplastbox]{flushend}
\usepackage{xcolor}
\usepackage{listings}
\usepackage{multirow}


% Always include hyperref last
\usepackage[bookmarks=true,breaklinks=true,letterpaper=true,colorlinks,linkcolor=black,citecolor=blue,urlcolor=black]{hyperref}
\usepackage[colorinlistoftodos,prependcaption,textsize=small]{todonotes}
% Ensure letter paper
\pdfpagewidth=8.5in
\pdfpageheight=11in

\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%


\newcommand{\proj}{\benchmark{TW}\xspace}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Figsub}[1]{Fig.~\subref{#1}}
\newcommand{\Tbl}[1]{Tbl.~\ref{#1}}
\newcommand{\Sec}[1]{Sec.~\ref{#1}}
\newcommand{\fixme}[1]{{\textcolor{red}{{#1}}}}
\newcommand{\benchmark}[1]{{\texttt{#1}}}
\renewcommand{\paragraph}[1]{\vspace*{0.05cm}\noindent\textbf{#1}\hspace*{.1cm}}
\newcommand{\FIXME}[2]{{\textcolor{red}{{#1} says: {#2}}}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
               \node[shape=circle,fill,inner sep=0.6pt] (char) {\textcolor{white}{#1}};}}
\lstset{frame=tb,
  language=C++,
  aboveskip=0mm,
  belowskip=0mm,
  showstringspaces=false,
  columns=flexible,
  %frame=L,
  numbers=left,
  numberstyle=\ttfamily\color{gray}\scriptsize,
  stepnumber=1,
  numbersep=1pt,
  basicstyle={\scriptsize\ttfamily},
  %basicstyle=\footnotesize,
  %keywordstyle=\color{blue},
  %commentstyle=\color{gray},
  %keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  %stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=2,
  escapeinside={(*@}{@*)}
}


% \def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
